ferret: a Framework for Benchmarking Explainers on Transformers

As Transformers are increasingly relied upon to solve complex NLP problems, there is an increased need for their decisions to be humanly interpretable. While several explainable AI (XAI) techniques for interpreting the outputs of transformer-based models have been proposed, there is still a lack of easy access to using and comparing them. We introduce ferret, a Python library to simplify the use and comparisons of XAI methods on transformer-based classifiers. With ferret, users can visualize and compare transformers-based models output explanations using state-of-the-art XAI methods on any free-text or existing XAI corpora. Moreover, users can also evaluate ad-hoc XAI metrics to select the most faithful and plausible explanations. To align with the recently consolidated process of sharing and using transformers-based models from Hugging Face, ferret interfaces directly with its Python library. In this paper, we showcase ferret to benchmark XAI methods used on transformers for sentiment analysis and hate speech detection. We show how specific methods provide consistently better explanations and are preferable in the context of transformer models.

==> intro_v1.tex <==

% Transformers are now consolidated as the standard de facto for many NLP applications. Their improving performance (and depleting intelligibility) attracted focused efforts on research for interpretability algorithms.

Recent work has interpreted Transformers using explainable AI (XAI) techniques on several NLP tasks \cite{10.1145/3546577}.
These studies used core XAI methods \cite{ribeiro2016should,NIPS2017_lundberg_SHAP,DBLP:journals/corr/SimonyanVZ13} or devised new approaches tailored to Transformer models \cite{wallace-etal-2019-universal,DBLP:journals/corr/LiMJ16a,jin2019towards,ross-etal-2021-explaining}.  

However, XAI for Transformers is mainly scattered and hard to operationalize. Methods come either with (independent) official implementations or framework-specific umbrella libraries, such as torch's Captum \cite{kokhlikyan2020captum}, that do not allow either evaluation or cross-method comparison. Further, existing implementations are not integrated with widespread Transformers libraries, such as Hugging Face's transformers \cite{wolf-etal-2020-transformers}.
The lack of standardization and weak interoperability leaves practitioners with unsolved questions, such as choosing the \textit{best} method given a task and a model \cite{attanasio-etal-2022-benchmarking}. 
%The lack of a standard way to produce and provide explanations and evaluate them across multiple explainers often leaves practitioners with unsolved questions, such as choosing the \textit{best} method given a task and a model \cite{attanasio-etal-2022-benchmarking}. 

% No unified framework bridging widespread Transformers libraries, such as Hugging Face's transformers \cite{wolf-etal-2020-transformers}, with easy explanation generation and benchmarking exists to date. 

%For example, consider the class of feature importance methods \cite{danilevsky-etal-2020-survey}. LIME~\cite{ribeiro2016should} estimates word importance by learning a regression model and presenting the user with the learned weights.
%\newcite{DBLP:journals/corr/SimonyanVZ13}, instead, impute word contributions measuring gradients with respect to the model's loss, i.e., how \textit{sensitive} is the model to each input component. 
%Current evidence shows that these differences are more than subtle \cite{attanasio-etal-2022-benchmarking}, motivating the need for a principled benchmarking framework to ultimately decide which method to prefer.

%Motivated by renewed requirements in regulation policies and social decision-making \cite{european_commission_regulation_2016, goodman2017european}, the issue of evaluating and benchmarking explanations has gained interest. 
%Recent works have discussed the properties of faithfulness, plausibility \cite{jacovi-goldberg-2020-towards}, and simulatability \cite{hase-bansal-2020-evaluating} of explanations. Others introduced new diagnostic benchmarks, datasets, and metrics to compare different interpretability methods \cite{atanasova-etal-2020-diagnostic,deyoung-etal-2020-eraser,attanasio-etal-2022-benchmarking}.
%However, these focused efforts show a common limitation: the authors devise and develop their study in \textit{technical isolation}, i.e., under no unified framework that allows either testing new explainers, new evaluation metrics, or datasets, ultimately hindering solid benchmarking. In other words, it is unnecessarily hard to answer paramount questions such as: Given all explanation methods applicable to my use case, \textit{which} one should I choose? Which method is more \textit{reliable}? Can I \textit{trust} it?

We introduce \placeholder,\footnote{\placeholder is a novel \textbf{f}ram\textbf{e}wo\textbf{r}k for benchma\textbf{r}king \textbf{e}xplainers on \textbf{T}ransformers.} an open-source Python library that drastically streamlines the use and comparison of core XAI methods on Transformers.
The library stems from vertical scientific contributions and focused engineering efforts.
On the one hand,
\placeholder provides the first-of-its-kind API (see Figure~\ref{fig:example_code}) to use and benchmark explanation methods along the established criteria of faithfulness and plausibility \cite{jacovi-goldberg-2020-towards}.
On the other hand,
it integrates seamlessly with \textit{transformers} \cite{wolf-etal-2020-transformers}, making it an easy add-on to existing Transformer-based pipelines and NLP tasks.
%\placeholder is an open-source Python library with multiple functionalities.
\placeholder exposes four state-of-the-art token attribution XAI methods, six evaluation metrics, and three interpretability datasets. Further, it offers abstract interfaces to foster future integration of methods, metrics, and datasets. 

We showcase \placeholder on sentiment analysis and hate speech detection case studies. Faithfulness and plausibility metrics highlight SHAP \cite{NIPS2017_lundberg_SHAP} as the most consistent explainer on single- and multiple-samples scenarios.

%We discuss the library and API conceptualization in Section~\ref{sec:library_design}, the most relevant technical nice-to-haves in Appendix \ref{app:technical_details}. 

%With \placeholder, we provide a principled evaluation framework combining state-of-the-art interpretability methods, metrics, and datasets with an easy-to-use, extensible, and transformers-ready \cite{wolf-etal-2020-transformers} interface. 

\paragraph{Contributions.} We release \placeholder, the first-of-its-kind benchmarking tool for post-hoc interpretability tightly integrated with Hugging Face's \textit{transformers}.
%\textbf{Evaluation API using as the input Hugging Face model names and free text} or interpretability corpora.
We release our code and documentation (\repo), a demo (\urldemo) and a video tutorial (\urlvideo).
%\footnote{We show \placeholder's main functionalities via a demo at  and a video tutorial at .}

%We compare \placeholder with several libraries and tools that empower interpretability in language technologies (Section \ref{sec:related_work}) and show how \placeholder supersets their peculiar functionalities while being the first to offer explicit \textbf{evaluation APIs}.
%Finally, we test \placeholder in the real-world scenario of evaluating interpretability methods on text classifiers for hate speech detection.
